A survey on Bayesian inference for Gaussian mixture model

Clustering has become a core technology in machine learning, largely due to its application in the field of unsupervised learning, clustering, classification, and density estimation. A frequentist approach exists to hand clustering based on mixture model which is known as the EM algorithm where the parameters of the mixture model are usually estimated into a maximum likelihood estimation framework. Bayesian approach for finite and infinite Gaussian mixture model generates point estimates for all variables as well as associated uncertainty in the form of the whole estimates' posterior distribution. The sole aim of this survey is to give a self-contained introduction to concepts and mathematical tools in Bayesian inference for finite and infinite Gaussian mixture model in order to seamlessly introduce their applications in subsequent sections. However, we clearly realize our inability to cover all the useful and interesting results concerning this field and given the paucity of scope to present this discussion, e.g., the separated analysis of the generation of Dirichlet samples by stick-breaking and Polya's Urn approaches. We refer the reader to literature in the field of the Dirichlet process mixture model for a much detailed introduction to the related fields. Some excellent examples include (Frigyik et al., 2010; Murphy, 2012; Gelman et al., 2014; Hoff, 2009). This survey is primarily a summary of purpose, significance of important background and techniques for Gaussian mixture model, e.g., Dirichlet prior, Chinese restaurant process, and most importantly the origin and complexity of the methods which shed light on their modern applications. The mathematical prerequisite is a first course in probability. Other than this modest background, the development is self-contained, with rigorous proofs provided throughout.

==> chapter-FMM0.tex <==
\chapter{Bayesian Mixture Model111}\label{chapter:review_bayesian_mixture_model111}


\section{Simple Simulation}
Simple test to state that why the condition of  $\max(\alpha_k, k\leqslant K) < D/2$ in \citet{rousseau2011asymptotic} is a too strong constriction. Test on simulated data with true cluster number $k_0$ = 3 clusters, means -3, 0, 3 (and -2, 0, 2) respectively, standard deviation 1, and 500 number of datas. And set the number of cluster to be $k$ = 4 in our test. And using the symmetric $\dirichlet(1/4, \ldots, 1/4)$ as the prior on weights. The result shows that the spread of data have a large influence on the shrinkage of the components.


\begin{figure}[!h]
  \includegraphics[width=\linewidth]{img/result_rousseau_n5000_p1_k0-3_k-4_spread-3/all-sampling.pdf}
  \caption{Test on 5000 number of datas, the means of the three clusters are (-3, 0, 3) respectively. Three cluster with high probability, one with small.  [ALL SAMPLES, WITHOUT BURN-IN AND THINING]}
  \label{fig:trace_4_n5000_k0-3_k-4_spread-3}
\end{figure}

\begin{figure}[!h]
  \includegraphics[width=\linewidth]{img/result_rousseau_n5000_p1_k0-3_k-4_spread-2/all-sampling.pdf}
  \caption{Test on 5000 number of datas, the means of the three clusters are (-2, 0, 2) respectively. One cluster with high probability, three with small.  [ALL SAMPLES, WITHOUT BURN-IN AND THINING]}
  \label{fig:trace_4_n5000_k0-3_k-4_spread-2}
\end{figure}



==> chapter-hyper-fbgmm.tex <==


\subsection{Introduction}


\subsection{Hyperprior on symmetric Dirichlet distribution}\label{sec:hyper_fbgmm_background}

\begin{figure}[h!]
\centering
  \includegraphics[width=5cm]{img/gmplots/bgmm_finite_with_hyper.pdf}
  \caption{A Bayesian finite GMM with hyperprior on concentration parameter.}
  \label{fig:gmm_finite_with_hyper_second_one_same_with_first_one}
\end{figure}


Inspired by \citet{rasmussen1999infinite} and further discussed by \citet{gorur2010dirichlet}, they introduced a hyperprior on symmetric Dirichlet distribution prior. We here put a vague prior of Gamma shape on the concentration parameter $\alpha$ and use the standard $\balpha$ setting where $\alpha_k = \alpha = \alpha_+/K$ for $k=1, \ldots, K$. 

\begin{equation}
\alpha | a, b \sim \gammadist(a, b) \Longrightarrow p(\alpha | a,b) \propto \alpha^{a-1} e^{-b\alpha}. 
\end{equation}

To get the conditioned posterior distributions on $\alpha$ we need to derive the conditioned posterior distributions on all the other parameters,. But for a graphical model, this conditional distribution is a function only of the nodes in the Markov blanket. In our case, the Bayesian finite Gaussian mixture model, a Directed acyclic graphical (DAG) model, the Markov blanket includes the parents, the children, and the co-parents, as shown in Figure \ref{fig:gmm_finite_with_hyper_second_one_same_with_first_one}. From this graphical representation, we can find the Markov blanket for each parameter in the model, and then figure out their conditional posterior distribution to be derived:
\begin{equation}
\begin{aligned}
p(\alpha | \bpi, a, b) &\propto p(\alpha | a,b) p(\bpi | \alpha) \\
					&\propto \alpha^{a-1} e^{-b\alpha} \frac{\Gamma(K \alpha)}{\prod_{k=1}^K \Gamma(\alpha)} \prod_{k=1}^K \pi_k^{\alpha-1} \\
					&= \alpha^{a-1} e^{-b\alpha} (\pi_1 \ldots \pi_K)^{\alpha-1} \frac{\Gamma(K\alpha)}{[\Gamma(\alpha)]^K}. 
\end{aligned}
\end{equation}


The following two theorems give the proof that the conditional posterior distribution of $\alpha$ is log-concave.

%% theorem 1: log concave
\begin{theorem}
Define 
\begin{equation}
G(x) = \frac{\Gamma(K x)}{[\Gamma(x)]^K}. 
\label{equation:gx_log_concave2}
\end{equation}

For $x > 0$ and an arbitrary positive integer $K$,  the function G is strictly log-concave. 
\end{theorem}\label{theorem:gx_log_concave2}

\begin{proof}

From \citet{abramowitz1966handbook} we get $\Gamma(Kx) = (2\pi)^{\frac{1}{2}(1-K)} K^{K x-\frac{1}{2} } \prod_{i=0}^{K-1}\Gamma(x + \frac{i}{K})$.  Then

\begin{equation}
\log G(x) = \frac{1}{2}(1-K) \log(2\pi) + (Kx - \frac{1}{2})\log K + \sum_{i=0}^{K-1} \log \Gamma(x + \frac{i}{K}) - K \log \Gamma(x)
\end{equation}
and
\begin{equation}
[\log G(x)]^\prime =K \log K + \sum_{i=0}^{K-1} \Psi(x + \frac{i}{K}) - K \Psi(x),
\end{equation}
where $\Psi(x)$ is the Digamma function, and

\begin{equation}
\Psi^\prime(x)  = \sum_{h=0}^\infty \frac{1}{(x+h)^2}. 
\label{equation:fbgmm_hyperprior_digamma_derivative2}
\end{equation}

Thus
\begin{equation}
[\log G(x)]^{\prime \prime} = \left[\sum_{i=0}^{K-1} \Psi^\prime(x + \frac{i}{K}) \right]- K \Psi^\prime(x) < 0, \quad (x>0). 
\end{equation}
The last inequality comes from (\ref{equation:fbgmm_hyperprior_digamma_derivative2}) and concludes the theorem. 

\end{proof}

This theorem is a general case of Theorem 1 in \citet{merkle1997log}. 

%%%%%% log concave 2
\begin{theorem}
In $p(\alpha | \bpi, a, b)$, when $a \geq 1$, $p(\alpha | \bpi, a, b)$ is log-concave
\end{theorem}

\begin{proof}
It is easy to verify that $ \alpha^{a-1} e^{-b\alpha} (\pi_1 \ldots \pi_K)^{\alpha-1} $ is log-concave when $a \geq 1$. In view of that the product of two log-concave functions is log-concave and Theorem \ref{theorem:gx_log_concave2}, it follows that $\frac{\Gamma(K\alpha)}{[\Gamma(\alpha)]^K}$ is log-concave. This concludes the proof.
\end{proof}

From the two theorems above, we can find the conditional posterior for $\alpha$ depends only on the weight of each cluster. The distribution $p(\alpha | \bpi, a, b)$ is log-concave, so we may efficiently generate independent samples from this distribution using Adaptive Rejection Sampling (ARS) technique \citep{gilks1992adaptive}.






